Toward Certified Robustness Against Real-World Distribution Shifts

We consider the problem of certifying the robustness of deep neural networks against real-world distribution shifts. To do so, we bridge the gap between hand-crafted specifications and realistic deployment settings by proposing a novel neural-symbolic verification framework, in which we train a generative model to learn perturbations from data and define specifications with respect to the output of the learned model. A unique challenge arising from this setting is that existing verifiers cannot tightly approximate sigmoid activations, which are fundamental to many state-of-the-art generative models. To address this challenge, we propose a general meta-algorithm for handling sigmoid activations which leverages classical notions of counter-example-guided abstraction refinement. The key idea is to "lazily" refine the abstraction of sigmoid functions to exclude spurious counter-examples found in the previous abstraction, thus guaranteeing progress in the verification process while keeping the state-space small. Experiments on the MNIST and CIFAR-10 datasets show that our framework significantly outperforms existing methods on a range of challenging distribution shifts.

==> tex/91proofs.tex <==
\iffalse
\section{Proofs in Section \ref{sec:certify}}

In this appendix, we provide proofs of the results stated in Section \ref{sec:certify}.  For ease of exposition, we restate each result before proving it.

\subsection{Proof of Theorem \ref{thm:soundness-of-bab}}

\begin{theorem}
$\bab$ is sound, if $\rlx$ and $\bound$ are sound, and $\branch$ is exhaustive.
\end{theorem}

\begin{proof}
Suppose $\bab$ is not sound, that is, given input problem $P$, either 1) $\bab$ returns $\robust$ but $P^\star < 0$, or 2) $\bab$ returns $\notrobust$ but $P^\star \geq 0$. 

The two cases are symmetric and we only prove the first case, where $\bab$ returns $\robust$ but $P^\star < 0$. This occurs only when one of the following three conditions is satisfied: 1) $\rlx(P)$ is not an over-approximation of $P$; 2) for certain sub-problem $P'$, the lowerbound $l$ computed by $\bound{\widetilde{P'}}$ is non-negative but $\widetilde{P'}^\star < 0$; 3) for all sub-problems $P'$ created by the $branch$ method, $P'^\star \geq 0$ but $P^\star < 0$. Condition 1) and 2) cannot occur when $\rlx$ and $\bound$ are sound. Recall that $\branch$ is exhaustive if given an optimization problem
$P$, $\branch$ returns a set of sub-problems $\mathcal{P}$ such that $P^\star = \min(\{P'^\star | P' \in \mathcal{P} \})$. Therefore, 3) cannot hold when $\branch$ is exhaustive.
\end{proof}


\subsection{Proof of Theorem \ref{thm:bab-sound-and-complete}}

\begin{theorem}
For ReLU neural networks, $\bab$ is sound and complete if $\rlx$ and $\bound$ are sound and complete, and $\branch$ performs ReLU splitting.
\end{theorem}

\begin{proof}
Since ReLU splitting is exhaustive, soundness follows from Theorem~\ref{thm:soundness-of-bab}.
Regarding completeness, in the worst case, the analysis of $P$ via convex relaxation (line 4-5) remains inconclusive until $P$ itself becomes convex (i.e., $\widetilde{P} = P$), which happens when $\branch$ has split on all ReLUs. Suppose there are $n$ ReLUs in the ReLU neural network. In the worst case, $\branch$ would create $2^n$ sub-problems, $\mathcal{P}$, each of which can be solved \emph{exactly} by $\bound$. The algorithm will return $\robust$ if $P^\star \geq 0$ for each $P \in \mathcal{P}$, or $\notrobust$ otherwise.
\end{proof}


\subsection{Proof of Proposition \ref{prop:lipschitz}}

\begin{proposition}
Let $x \in\calX$ and assume that for a fixed $z \sim p(z|x)$, the instance $\bar{x} \triangleq G(x, z)$ is classified by $C$ as belonging to the class $i^\star$.  Then assuming that the map $z\mapsto f(G(x, z))$ is locally $L$-Lipschitz in the $\ell_2$ norm, it follows that $C(G(x, z)) = C(G(x, z'))$ $\forall z'$ such that $\norm{z - z'} \leq \delta^\star$, where
%
\begin{align}
    \delta^\star = (1/L\sqrt{2}) \: \min_{1\leq j\leq k, \: j\neq i^\star} \: \left| f_j(G(x, z)) - f_{i^\star}(G(x, z))\right|.\label{eq:lipschitz-delta-app}
\end{align} 
\end{proposition}

\begin{proof}
The proof of this proposition closely follows the proof of Proposition 1 in~\cite{fazlyab2019efficient}.  The main difference is that the result is applied to the compositional architecture $f\circ G$.

To begin, let $i^\star$ be the predicted class for $\bar{x} = f(G(x,z))$, i.e.
%
\begin{align}
    i^\star = \argmax_{1\leq i\leq k} f_k(G(x, z)).
\end{align}
%
We next define $\calP_{i^\star}$ to be the set of all output vectors in $\R^k$ which yield the highest score for the label $i^\star$; more formally, $\calP_{i^\star}$ can be defined as the following polytope:
%
\begin{align}
    \calP_{i^\star} \triangleq \left\{ y\in\R^k : (e_j - e_{i^\star})^\top y \leq 0 \quad\text{for }j \text{ s.t. } 1\leq j\leq k, \: j\neq i^\star\right\}.
\end{align}
%
By construction, $f(G(x,z)) \in\calP_{i^\star}$.  Furthermore, the distance from $f(G(x,z))$ to the boundary $\partial \calP_{i^\star}$ of the polytope $P_{i^\star}$ is the minimum distance from $f(G(x,z))$ to any of the edges of the polytope:
%
\begin{align}
    \dist(f(G(x,z)), \partial \calP_{i^\star}) &= \inf_{y\in\partial \calP_{i^\star}} \norm{y - f(G(x,z))}_2 \\
    &= \frac{1}{\sqrt{2}} \min_{1\leq j\leq k, \: j\neq i^\star} |f_j(G(x,z)) - f_{i^\star}(G(x,z))|.
\end{align}
%
Now assuming that $z\mapsto f(G(x,z))$ is $L$-Lipschitz in the $\ell_2$ norm, we know that
%
\begin{align}
    \dist(f(G(x,z)), f(G(x, z'))) &= \norm{f(G(x,z)) - f(G(x,z'))}_2 
    \\
    &\leq L\delta
\end{align}
%
$\forall z'$ such that $\norm{z - z'}_2 \leq \delta$.  Now let $\delta^\star$ be defined as in \eqref{eq:lipschitz-delta-app}.  Observe that for this choice of the radius $\delta^\star$, it follows that
%
\begin{align}
    \dist(f(G(x,z)), f(G(x,z'))) \leq \dist(f(G(x,z)), \partial \calP_{i^\star})
\end{align}
%
$\forall z'$ such that $\norm{z - z'}_2 \leq \delta^\star$.  Therefore, the output will not change for perturbations bounded by $\delta^\star$ in the latent variable $z$.  This completes the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:lipschitz}}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{img/lip-arch.png}
    \caption{\textbf{Compositional architecture for Lipschitz estimation.}}
    \label{fig:lip-arch}
\end{figure}

\begin{theorem}
Let $\mathbb{S}^n$ denote the $n$-dimensional positive semidefinite cone, where $n$ is the total number of neurons in $f\circ G$, and assume that each activation function in $f\circ G$ is slope-restricted in the sector $[\alpha, \beta]$.  Define the set $\mathcal{T}_n := \{ T\in\mathbb{S}^n \: | \: T = \sum\nolimits_{i=1}^n \lambda_{i} e_ie_i^\top, \: \lambda_{i} \geq 0 \}$.  Define linear map
\begin{align}
    M(\rho, T) := \begin{bmatrix}
        A \\ B
    \end{bmatrix}^\top \begin{bmatrix}
        -2\alpha\beta T & (\alpha + \beta)T \\
        (\alpha + \beta)T & -2T
    \end{bmatrix} \begin{bmatrix}
        A \\ B
    \end{bmatrix} + \begin{bmatrix}
        -\rho I & 0 & \hdots & 0 \\
        0 & 0 & \hdots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \hdots & W^\top W
    \end{bmatrix}
\end{align}
%
where $A$ and $B$ are matrices depending only on the fixed input $x$ and the weight matrices of $f$ and $G$, and $W$ is the final weight matrix of $f$.  Assuming that there exists a $\rho > 0$ such that $M(\rho,T) \preceq 0$ holds for some $T\in T_n$, then $\sqrt{\rho}$ is a local Lipschitz constant for the map $z\mapsto f(G(x,z))$.
\end{theorem}

\begin{proof}
The main idea in this proof is to manipulate the form of the architecture $f\circ G$ such that it resembles the feed-forward structure used in~\cite{fazlyab2019efficient}.  After this manipulation, the result directly follows from Theorem 2 in~\cite{fazlyab2019efficient}.

\textbf{Step 1: A general architecture for Lipschitz estimation.}  To prove this theorem, we first make concrete the general form of the architecture of $f\circ G$.  In particular, consider the compositional architecture for $f\circ G$ in Figure~\ref{fig:lip-arch}.  The leftmost blocks (shown in yellow) comprise the generator $G(x,z)$ and the rightmost block (shown in red) is the classifier $f(x)$.  In each block, we write the weight matrices $W$ and bias vectors $b$ in the corresponding blocks.  Thus, the branch at the top left that encodes $x$ to the intermediate activation vector $a_x$ via the weight matrices $\{(W_x^{(i)}, b_x^{(i)})\}_{i=1}^{N_x}$ represents the following transformation:
%
\begin{align}
    x^{(1)} = x, \quad x^{(k+1)} = \phi\left(W_x^{(k)}x^{(k)} + b_x^{(k)}\right) \quad\forall k\in[N_x-1], \quad a_x = \phi(W_x^{(N_x)}x^{(N_x)} + b_x^{(N_x)})
\end{align}
%
where $[n] := \{1, \dots, n\}$ and $\phi$ is applied coordinate-wise via
%
\begin{align}
    \phi(x) = \begin{bmatrix} \varphi(x_1) & \cdots & \varphi(x_n) \end{bmatrix}^\top
\end{align}
%
where $\varphi:\R\to\R$ is a slope-restricted activation function.  The transformations for the other sets of weight matrices can all be written similarly.  That is, the map from $z$ to $a_z$ can be written as
%
\begin{align}
    z^{(1)} = z, \quad z^{(k+1)} = \phi\left(W_z^{(k)}z^{(k)} + b_z^{(k)}\right) \quad\forall k\in[N_z-1], \quad a_z = \phi(W_z^{(N_z)}z^{(N_z)} + b_z^{(N_z)});
\end{align}
%
the map from $\begin{bmatrix} a_x & a_z\end{bmatrix}^\top$ to $\bar{x}$ can be written as
%
\begin{align}
    a^{(1)} = \begin{bmatrix} a_x \\ a_z\end{bmatrix}, \quad a^{(k+1)} = \phi\left(W_G^{(k)}a^{(k)} + b_G^{(k)}\right) \:\: \forall k\in[N_G-1], \:\: \bar{x} = \phi(W_G^{(N_G)}a^{(N_G)} + b_G^{(N_G)});
\end{align}
%
and the map from $\bar{x}$ to $y$ can be written as
%
\begin{align}
    \bar{x}^{(1)} = \bar{x}, \quad \bar{x}^{(k+1)} = \phi\left(W_f^{(k)}\bar{x}^{(k)} + b_f^{(k)}\right) \quad\forall k\in[N_f-1], \quad y = W_f^{(N_f)}\bar{x}^{(N_f)} + b_f^{(N_f)}.
\end{align}

\textbf{Step 2: Compactly expressing $f\circ G$.}
Of immediate interest is to write down these equations in a more condensed form.  Notably, as we are only interested in a local Lipschitz constant for a fixed $x\in\calX$, we can absorb the vector $a_x$ into the bias term $b_G^{(1)}$.  Using this insight, we can write the end-to-end architecture using the following compact notation:
%
\begin{align}
    B\mathbf{z} = \phi(A\mathbf{z} + b) \quad\text{and}\quad y = D\mathbf{z} + b_f^{(N_f)} \label{eq:compact-notation}
\end{align}
%
for matrices $A$, $B$, $D$, and $b$ depending on the weight matrices and bias vectors described above.  To define these matrices, we define the following notation:
%
\begin{align}
    W_z &:= \textbf{diag}\left(W_z^{(1)}, \dots, W_z^{(N_z)}\right) \\
    W_G &:= \textbf{diag}\left(W_G^{(1)}(\texttt{:}, \: \textbf{dim}(a_x)\text{:}), W_G^{(2)}, \dots, W_G^{(N_G)}\right) \\
    W_f &:= \textbf{diag}\left(W_f^{(1)}, \dots, W_f^{(N_f-1)}\right)
\end{align}
%
where
%
where $W_G^{(1)}(\texttt{:}, \: \textbf{dim}(a_x)\texttt{:})$ denotes the final $\textbf{dim}(a_z)$ columns of $W_G^{(1)}$.  Given this notation, we can now define the following matrices:
%
\begin{align}
    &A := \begin{bmatrix}
        W_z & 0 & 0 & 0 & 0\\
        0 & W_G & 0 & 0 & 0\\
        0 & 0 & W_g & 0 & 0 \\
        0 & 0 & 0 & W_f & 0 \\ 
    \end{bmatrix}, \quad B:= \begin{bmatrix} 
        0 & I & 0 & 0 & 0 \\
        0 & 0 & I & 0 & 0 \\
        0 & 0 & 0 & I & 0 \\
        0 & 0 & 0 & 0 & I \\
    \end{bmatrix}, \label{eq:a-and-b} \\
    &D := \begin{bmatrix}
        0 & \cdots & 0 & W_f^{(N_f)}
    \end{bmatrix}, \\
    &b = \begin{bmatrix}
        b_z^{(1)} &
        \cdots &
        b_z^{(N_z)} &
        \tilde{b}_G^{(1)} &
        b_G^{(2)} &
        \cdots &
        b_G^{(N_G)} &
        b_f^{(1)} &
        \cdots &
        b_f^{(N_f-1)}
    \end{bmatrix}^\top 
\end{align}
%
where $\tilde{b}_G^{(1)} = b_G^{(1)} + W_G^{(1)}(\texttt{:}, \: \texttt{:}\textbf{dim}(a_x))a_x$.   Note that $B$ is defined so that it has the same number of columns as $A$.

\textbf{Step 3: Finish the proof.} The utility of the notation in \eqref{eq:compact-notation} is that it provides us a compact way to express the neural network by leveraging the fact that the slope-restricted activation is applied coordinate-wise.  Moreover, this notation is consistent with the network architecture considered in equation (2) in~\cite{fazlyab2019efficient}.  To this end, as the activation function $\varphi$ is assumed to be slope-restricted, we can leverage Theorem 2 in~\cite{fazlyab2019efficient} to derive the statement of the theorem.  Thus, letting the matrices $A$ and $B$ be defined as in \eqref{eq:a-and-b}, we consider the matrix inequality %
\begin{align}
    M(\rho, T) := \begin{bmatrix}
        A \\ B
    \end{bmatrix}^\top \begin{bmatrix}
        -2\alpha\beta T & (\alpha + \beta)T \\
        (\alpha + \beta)T & -2T
    \end{bmatrix} \begin{bmatrix}
        A \\ B
    \end{bmatrix} + \begin{bmatrix}
        -\rho I & 0 & \hdots & 0 \\
        0 & 0 & \hdots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \hdots & (W_f^{(N_f)})^\top W_f^{(N_f)}
    \end{bmatrix} \preceq 0 \label{eq:matrix-inequal}
\end{align}
%
By Theorem 2 in~\cite{fazlyab2019efficient}, if \eqref{eq:matrix-inequal} is satisfied for some $(\rho, T)\in\R_{\geq 0}\times \mathcal{T}_n$, then
%
\begin{align}
    \norm{f(G(x,z)) - f(G(x,z'))}_2 \leq \sqrt{\rho} \norm{z - z'}_2 \quad\forall z, z'.
\end{align}
%
In other words, the map $z\mapsto f(G(x,z))$ is $\sqrt{\rho}$-Lipschitz continuous.  This completes the proof.
\end{proof} 

\fi

==> tex/alg.tex <==
\begin{wrapfigure}{r}{0.48\textwidth}
\begin{minipage}[t]{6.5cm} 
\vspace{-8mm}
\begin{algorithm}[H]
\small
\begin{algorithmic}[1]
  \State {\bfseries Input:} constraints $S(u)$ and objective $g(u)$
  \State {\bfseries Output:} \robust{} if $\min g_S \ge 0$
  \Function{$\bab$}{$S, g$}
  \State {$\widetilde{g}_S = \rlx(S, g)$ }
  \State {$l, \alpha$ = $\bound(\widetilde{g}_S)$ }
  \If{$l > 0$}
  \State {\bf return} \robust{}
  \ElsIf{$S(\alpha) \land g(\alpha) < 0$}
  \State {\bf return} \notrobust{}
  \EndIf
  \For {$S' \in \branch(S, g)$}
  \If {$\neg\bab(S', g)$}
  \State {\bf return \notrobust{}} 
  \EndIf
  \EndFor
  \State {\bf return} \robust
  \EndFunction
\end{algorithmic}
\caption{Complete local verification.\label{alg:bab}}
\end{algorithm}
\end{minipage}
\end{wrapfigure}


==> tex/arch.tex <==
\begin{wrapfigure}{r}{0.48\textwidth}
\begin{minipage}[t]{6.5cm} 
% \vspace{-2mm}
\vspace*{1mm}
\setlength\tabcolsep{5pt}
\centering		
\sffamily
\scriptsize
\begin{tabular}{lllcc}
\toprule
Dataset & Model & Type & \# ReLUs  & \# Layers \\ 
\cmidrule(lr){1-5}
\multirow{3}{*}{\vspace*{0pt}MNIST}   & Prior & FFNN &  1084      &  2  \\
& Gen.  & FFNN &  850       &  1  \\
& Class. & FFNN &  320       &  2 \\
\cmidrule(lr){1-5}
\multirow{3}{*}{\vspace*{0pt}CIFAR10} & Prior      & FFNN &  3372      &  2 \\
        & Gen.  & Conv.   &  8192      &  2 \\
        & Class. & Conv.   &  2568      &  4\\ 
\bottomrule
\end{tabular}
% \vspace{-1.5mm}
\caption{Architectures overview \label{tab:architectures}}
\end{minipage}
% \vspace{-2mm}
\end{wrapfigure}


==> tex/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section X.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Sec.~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See App.~\ref{app:proofs}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will make the implementation, the benchmark, as well as an artifact to reproduce the results publicly available after the paper goes public.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See App.~\ref{app:cvae}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Sec.~\ref{sec:experiments} and App.~\ref{app:cvae}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See App.~\ref{app:license}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> tex/images.tex <==
\begin{figure}[t!]
\vspace{-1cm}
\begin{minipage}{0.6\textwidth}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/brightness_ind3_target6_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/contrast_ind39_target8_theta0.5_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/gaussian-blur_ind95_target8_theta1.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/rotation_ind21_target5_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=\linewidth]{img/scale_ind30_target5_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=\linewidth]{img/shear_ind54_target0_theta2.0_orig.png}  
\end{subfigure}

\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=\linewidth]{img/brightness_ind3_target6_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/contrast_ind39_target8_theta0.5_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/gaussian-blur_ind95_target8_theta1.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/rotation_ind21_target5_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/scale_ind30_target5_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/shear_ind54_target0_theta2.0_adv.png}  
\end{subfigure}
\end{minipage}
\hfill
\hspace{-6mm}
\begin{minipage}{0.48\textwidth}
\centering
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_brightness_ind10_target4_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_contrast_ind166_target0_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_fog_ind46_target5_theta2.0_orig.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_gaussian_ind92_target1_theta2.0_orig.png}  
\end{subfigure}

\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_brightness_ind10_target4_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_contrast_ind166_target0_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_fog_ind46_target5_theta2.0_adv.png}  
\end{subfigure}
\begin{subfigure}{1.3cm}
\centering
  % include first image
\includegraphics[width=1\linewidth]{img/cifar10_gaussian_ind92_target1_theta2.0_adv.png}  
\end{subfigure}
\end{minipage}
\caption{Counter-examples found in the perturbation set by the verifier. Perturbations on MNIST (from left to right): brightness, contrast, gaussian blur, rotation, scale, sheer. Perturbations on CIFAR (from left to right): brightness, contrast, fog, gaussian blur.\label{fig:counter-examples}}
\vspace{1.5cm}
\end{figure}


==> tex/refinement_03.tex <==
\begin{tikzpicture}[scale=0.35,
declare function={
    sig(\x) = 1 / (1 + exp(-\x));
    sig_prime(\x) = {(1 / (1+exp(-\x))) * (1 - (1 / (1+exp(-\x))))};
},
]
\begin{axis}%
[
    % grid=major,     
    xmin=-5,
    xmax=5,
    axis x line=bottom,
    ytick = none,
    grid = none,
    ymax=1,
    ymin=0,
    axis y line=middle,
    xlabel={$n^b$},
    ylabel={$n^a$},
    xlabel style={at={(ticklabel* cs:1)},anchor=south, font=\Large\boldmath},
    ylabel style={at={(ticklabel* cs:1)},anchor=south, font=\Large\boldmath},
    xtick = {-2, 4},
    xticklabels = {$l$,$u$},
    tick label style={black, font=\boldmath},
    tick align=outside,
]

    \addplot%
    [
        black,%
        mark=none,
        samples=100,
        domain=-6:6,
    ]
    {sig(x)};

    \addplot%
    [
        gray,%
        mark=none,
        samples=100,
        domain=0:4,
        dashed,
    ]
    {sig_prime(4)*(x-4) + sig(4)};

    \addplot%
    [
        green,%
        mark=none,
        samples=100,
        domain=-1:4,
    ]
    {sig_prime(4)*(x-(-1)) + sig(-1)};

    \addplot%
    [
        green,%
        mark=none,
        samples=100,
        domain=-4:-1,
    ]
    {sig_prime(-1)*(x-(-1)) + sig(-1)};
    
    \addplot%
    [
        black,%
        dashed,
        mark=none,
        samples=100,
    ]
    coordinates {(-1, 0.15) (-1, sig(-1))};

    \addplot%
    [
        black,%
        dashed,
        mark=none,
        samples=100,
    ]
    coordinates {(4, 0) (4, sig(4))};

    \addplot%
    [
        black,%
        dashed,
        mark=none,
        samples=100,
    ]
    coordinates {(-3, 0) (-3, sig(-3))};
    

    \addplot%
    [
        black,%
        dashed,
    ]
    coordinates {(-2, 0.5)};
    
    \addplot [only marks,mark=*,red] coordinates { (-1,0.15) };
    \node at (axis cs:-1,0.13) [anchor=north, font=\boldmath] {$(p, q)$};
\end{axis}
\end{tikzpicture}
